ForestFirewalls: Getting Firewall Configuration Right in Critical Networks (Technical Report)

Firewall configuration is critical, yet often conducted manually with inevitable errors, leaving networks vulnerable to cyber attack [40]. The impact of misconfigured firewalls can be catastrophic in Supervisory Control and Data Acquisition (SCADA) networks. These networks control the distributed assets of industrial systems such as power generation and water distribution systems. Automation can make designing firewall configurations less tedious and their deployment more reliable. In this paper, we propose ForestFirewalls, a high-level approach to configuring SCADA firewalls. Our goals are three-fold. We aim to: first, decouple implementation details from security policy design by abstracting the former; second, simplify policy design; and third, provide automated checks, pre and post-deployment, to guarantee configuration accuracy. We achieve these goals by automating the implementation of a policy to a network and by auto-validating each stage of the configuration process. We test our approach on a real SCADA network to demonstrate its effectiveness.

==> abstract.tex <==
\begin{abstract}
Firewall configuration is critical, yet often conducted manually with inevitable errors, leaving networks vulnerable to cyber attack \cite{wool2004}. The impact of misconfigured firewalls can be catastrophic in \ac{SCADA} networks. These networks control the distributed assets of industrial systems such as power generation and water distribution systems. Automation can make designing firewall configurations less tedious and their deployment more reliable. 

In this paper, we propose \textit{ForestFirewalls}, a high-level approach to configuring \ac{SCADA} firewalls. Our goals are three-fold. We aim to: first, decouple implementation details from security policy design by abstracting the former; second, simplify policy design; and third, provide automated checks, pre and post-deployment, to guarantee configuration accuracy. We achieve these goals by automating the implementation of a policy to a network and by auto-validating each stage of the configuration process. We test our approach on a real SCADA network to demonstrate its effectiveness.
\end{abstract}

%% Word count is at most 200 words
%% Current count 198 words

%approach to configuring \ac{SCADA} firewalls
